Time-Periodic Solutions of a Driven--Damped $\phi^4$ Equation on Bounded Domains

We prove the existence of time-periodic solutions for a driven--damped $\phi^4$ wave equation posed on a bounded spatial domain with periodic boundary conditions. The result is obtained at the level of the full partial differential equation. The analysis is based on a Lyapunov--Schmidt decomposition in a time-periodic function space. A key structural feature is the presence of linear damping, which ensures uniform invertibility of the associated linear operator on the complement of the kernel and removes the need for nonresonance conditions. After introducing a truncation to control the cubic nonlinearity, we solve the complement equation via a contraction mapping argument and reduce the problem to a scalar kernel equation. The latter is treated using a mean/zero-mean decomposition and a fixed-point argument. A period-averaged energy estimate then allows one to remove the truncation and obtain a time-periodic weak solution under explicit smallness conditions on the forcing parameters

==> sec_conclusions.tex <==
\section{Conclusion}
\label{sec_conclusions}

In this work we have established a fully rigorous, PDE-level existence theory for
time-periodic solutions of a driven--damped $\phi^4$ field equation on a bounded
spatial domain.
Adapting the Lyapunov--Schmidt framework of Fe\v{c}kan to the present setting,
we decomposed the dynamics into the kernel of the spatial operator and its
orthogonal complement, proved uniform invertibility of the associated damped
time-periodic linear operator, and solved the complement equation by a contraction
mapping argument after a standard truncation.
This reduction led to a finite-dimensional kernel equation whose solvability,
together with an explicit energy identity and a period-averaged dissipation
balance, allowed us to remove the cut-off and obtain a genuine $T$-periodic
solution of the original PDE.

Beyond the existence result itself, the analysis highlights the decisive role
played by bounded spatial domains.
Finite intervals endowed with boundary conditions discretize the spatial spectrum,
which is precisely the structural ingredient required for Fourier--spectral
inversion estimates and the absence of small-divisor obstructions.
In the presence of damping, this yields a particularly transparent and robust
route to time-periodic solutions under mild smallness assumptions on the forcing.
From this perspective, the theorem provides a rigorous explanation of why
finite-interval numerical simulations naturally exhibit stable time-periodic
responses in driven nonlinear field equations.

At the same time, the scope of the result is clearly delineated.
The periodic-boundary-condition framework developed here does not directly address
the existence of periodically moving single kinks on the real line, since such
solutions are not compatible with periodic spatial boundary conditions and require
a fundamentally different decomposition based on the linearization about kink
manifolds.
Rather than replacing collective-coordinate approaches, the present analysis
provides a complementary PDE-level foundation that clarifies the mathematical
mechanisms underlying bounded-domain computations and reduced descriptions.

Finally, the structure of the proof points naturally toward further extensions.
On finite intervals with Dirichlet or mixed boundary conditions, the same strategy
applies after replacing the kernel decomposition by a spectral-gap splitting onto
low spatial modes, leading to an even simpler reduction without a genuine kernel.
More ambitiously, one may seek to extend the Lyapunov--Schmidt framework to the
kink sector by decomposing around a moving kink manifold and imposing suitable
orthogonality conditions to isolate translational and internal modes.
Such an approach would yield a rigorously justified modulation system for kink
dynamics coupled to a controlled radiation component, thereby bridging the gap
between Fe\v{c}kan-type PDE analysis and collective-coordinate theories of driven
kinks.


